Semantic Equivariant Mixup

Mixup is a well-established data augmentation technique, which can extend the training distribution and regularize the neural networks by creating ''mixed'' samples based on the label-equivariance assumption, i.e., a proportional mixup of the input data results in the corresponding labels being mixed in the same proportion. However, previous mixup variants may fail to exploit the label-independent information in mixed samples during training, which usually contains richer semantic information. To further release the power of mixup, we first improve the previous label-equivariance assumption by the semantic-equivariance assumption, which states that the proportional mixup of the input data should lead to the corresponding representation being mixed in the same proportion. Then a generic mixup regularization at the representation level is proposed, which can further regularize the model with the semantic information in mixed samples. At a high level, the proposed semantic equivariant mixup (sem) encourages the structure of the input data to be preserved in the representation space, i.e., the change of input will result in the obtained representation information changing in the same way. Different from previous mixup variants, which tend to over-focus on the label-related information, the proposed method aims to preserve richer semantic information in the input with semantic-equivariance assumption, thereby improving the robustness of the model against distribution shifts. We conduct extensive empirical studies and qualitative analyzes to demonstrate the effectiveness of our proposed method. The code of the manuscript is in the supplement.

==> 5_theory.tex <==
In this section, we provide a theoretical understanding of how semantic supervision helps to learn good representation. Our analysis first explore the connection between semantic supervision and good representation. Then we show how \textsc{SEM} helps to obtain a good representation. To introduce the theoretical framework, we first present the basic settings.

\textbf{Basic settings.} Normally, for certain class $p$, we'll assume the distribution of the representation of samples from class $p$ with mean $\mu_p$ and covariance $\Sigma_p$. For most of time, we'll further assume a Gaussian distribution $\mathcal{N}(\mu_p,\Sigma_p)$. When applying Mixup, we obtain mixed samples $\widetilde{x}_{i,j} = \lambda x_i + (1 - \lambda) x_j (\lambda \in (0 , 1))$ with $x_i,x_j \in$ class $p,q$ and its corresponding representation $r_{(x_i,x_j)}$. For fixed $\lambda$, we also assume $r_{(x_i,x_j)}$ from a distribution with mean $\mu_p$ and covariance $\Sigma_{p,q}$. Note that when $p \neq q$, we actually get a synthesised distribution.


\textbf{Semantic supervision. } It's hard to define what a good representation is. But we can always say that \textit{For samples $x_i$ and $x_j$ from the same class $p$, their representation $r_i$ and $r_j$ should be as close as possible.} To achieve that, we can choose a representative element $r_p$ and make all representations of class $p$ close to $r_{p}$. Specifically, we can chose $\mu_p$ as $r_p$. Formally, for a certain sample $x$ from class $p$ with representation $x_p$, we can define the process as follows, 

$$\min \mathbb{E}_\mathcal{D}[\mathrm{dissimilarity}(\mu_{p}, r_x)] $$

We define the above formula as Generalized Semantic Supervision (GSS). Combining GSS and  normal loss function, our final optimization objective is

$$\min \mathbb{E}_\mathcal{D}[\ell[f(x) , y] + \alpha \times \mathrm{dissimilarity}(\mu_{p}, r_x)] $$

where $\alpha$ is a hyperparameter controlling how Semantic supervision affects the result.

For mixup-based method with samples $x_i$ and $x_j$, we can rewrite the objective as 

$$\min  \mathbb{E}_\mathcal{\widetilde{D}}[\ell[f(\tilde{x} ) , \tilde{y}] + \alpha \times \mathrm{dissimilarity}(r_{(x_i,x_j)} , \mu_{p,q})] $$

Now the key problem is that no matter for non-mixup nor for mixup, we have no idea of what $\mu_p$ or $\mu_{p,q}$ is. Obviously,  we need to find an unbiased estimator $\hat{\mu_{p,q}}$ (or $\hat{\mu_{p}}$) of $\mu_{p,q}$ with $\mathrm{MSE}(\hat{\mu_{p,q}})=\mathbb{E}_\mathcal{\widetilde{D}}[(\hat{\mu_{p,q}}-\mu_{p,q})^2]$ as small as possible. For vanilla mixup, it can be seen that we can use $r_{(x_i,x_j)}$ as the estimator. However, when using $r_{(x_i,x_j)}$ as the estimator, the GSS term identically equals to zero and loses it function. So the goal of \textsc{SEM} is actually find another unbiased estimator with no less effect and keeps the GSS term not zero.

\textbf{Theorem 1. } \textit{Suppose we mix samples $x_i,x_j$ from class $p$ and $q$ with representation $r_{x_i} , r_{x_j} \in R^n$. The representation $r_{(x_i,x_j)}$ of the synthesised sample $\tilde{x}=\lambda x_1+(1-\lambda)x_2$ comes from distribution $P(\mu_{p,q},\Sigma_{p,q})$. We set $M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]=\lambda r_{x_i}+(1-\lambda)r_{x_j}$. According to \textit{semantic-equivariance assumption} , we have}

\begin{equation}
\begin{split}
\mathbb{E}_\mathcal{\widetilde{D}}[ M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]] &= \mathbb{E}_\mathcal{\widetilde{D}}[r_{(x_i,x_j)}]=\mu_{p,q}\\
\mathbb{E}_\mathcal{\widetilde{D}}[ ||M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}] - \mu_{p,q}||^2_2 ] &= \mathbb{E}_\mathcal{\widetilde{D}}[ ||r_{(x_i,x_j)} - \mu_{p,q}||^2_2 ]
\end{split}
\end{equation}

Theorem 1 shows that $M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]$ is an unbiased estimator of $\mu_{p,q}$ with effect no worse than $r_{(x_i,x_j)}$. Theorem 1 discuss the effect of $M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]$ on a general situation. Moreover, when $p=q$, according to \textit{label-equivariance assumption}, the synthesised sample $\hat{x}$ is also a member of class $p$. Under this situation, we now need to estimate $\mu_p$ of a real distribution $P(\mu_p,\Sigma_p)$. We can notice that when not using Mixup, we use $r_{x_i}(r_{x_j}) $ to estimate $\mu_p$, which, like $r_{(x_i,x_j)}$ also makes the SSG term zero.

\textbf{Theorem 2. } \textit{When $p=q$, comparing two estimators $r_{x_i}(r_{x_j}) $ and $M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]$, we have}

$$\mathbb{E}_\mathcal{\widetilde{D}}[ ||M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}] - \mu_{p}||^2_2 ] \leq \mathbb{E}_\mathcal{\widetilde{D}}[ ||r_{x_i}(r_{x_j}) - \mu_{p}||^2_2 ]$$

Theorem 2 tells us that when approximating a real distribution, \textsc{SEM} outperforms methods without Mixup. To sum up, we can tell that \textsc{SEM} is a good estimator no matter on real distribution or synthesised distribution. So we use $M_{\lambda}^{\mathcal{R}}[r_{x_i},r_{x_j}]$ and take dissimilarity as $\ell_2$ loss, we can get the final objective identical to Eq.~\ref{eq:semloss}.

